MaskingDepth: Masked Consistency Regularization for Semi-supervised Monocular Depth Estimation

We propose MaskingDepth, a novel semi-supervised learning framework for monocular depth estimation to mitigate the reliance on large ground-truth depth quantities. MaskingDepth is designed to enforce consistency between the strongly-augmented unlabeled data and the pseudo-labels derived from weakly-augmented unlabeled data, which enables learning depth without supervision. In this framework, a novel data augmentation is proposed to take the advantage of a naive masking strategy as an augmentation, while avoiding its scale ambiguity problem between depths from weakly- and strongly-augmented branches and risk of missing small-scale instances. To only retain high-confident depth predictions from the weakly-augmented branch as pseudo-labels, we also present an uncertainty estimation technique, which is used to define robust consistency regularization. Experiments on KITTI and NYU-Depth-v2 datasets demonstrate the effectiveness of each component, its robustness to the use of fewer depth-annotated images, and superior performance compared to other state-of-the-art semi-supervised methods for monocular depth estimation. Furthermore, we show our method can be easily extended to domain adaptation task. Our code is available at https://github.com/KU-CVLAB/MaskingDepth.

==> Table/5_table.tex <==
\begin{table}[t]
\centering
\resizebox{0.65\linewidth}{!}{%
\begin{tabular}{c|c|c|c}
        \toprule
        Method & Blocks &  AbsRel $\downarrow$ & \textbf{$\delta$}$\uparrow$ \\
        \midrule
        w/o head       &- &0.317 &0.423\\
        Transformer    &1 &0.125 &\textbf{0.856}\\
        Transformer    &2 &0.129 &0.848\\
        MLP            &2 &\textbf{0.124} &0.855\\
        \bottomrule
\end{tabular}
}\vspace{-10pt}
\caption{\textbf{Comparison of using different predictor head.}}
\label{tab:predictor}\vspace{-5pt}
\end{table}


==> Table/6_table.tex <==
\begin{table}[t!]
\centering
\resizebox{0.65
\linewidth}{!}{
\begin{tabular}{l|ccc}
        \toprule
        $K$ & AbsRel $\downarrow$ & RMSE $\downarrow$ &\textbf{$\delta$}$\uparrow$ \\
        \midrule
        $K=4$  &0.131 & 4.456 &0.850\\
        $K=16$ &0.128 & 4.298 &\textbf{0.855}\\
        $K=64$ &\textbf{0.124} & \textbf{4.263} &\textbf{0.855}\\
        $K=128$ &0.132 & 4.382 &0.849\\
        \bottomrule
\end{tabular}%
}\vspace{-5pt}
\caption{\textbf{Influence of the number of $K$.}}
\label{tab:numberK}\vspace{-5pt}
\end{table}
